Escrows are optics

We provide a categorical interpretation for escrows, i.e. trading protocols in trustless environment, where the exchange between two agents is mediated by a third party where the buyer locks the money until they receive the goods they want from the seller. A simplified escrow system can be modeled as a certain kind of morphism in the category of optics on a monoidal category. When objects in the base category have monoid and comonoid structures, more involved kinds of escrows `with intermediaries' can be modelled as morphisms with action-like properties.

==> fouche/alphabets.tex <==
\ExplSyntaxOn

\clist_new:N \g_fouche_upper_clist
\clist_gset:Nn \g_fouche_upper_clist { A,B,C,D,E,G,H,I,J,K,L,M,N,O,P,Q,R,T,U,V,W,X,Y,Z }

\clist_new:N \g_fouche_lower_clist
\clist_gset:Nn \g_fouche_lower_clist { a,b,c,d,e,g,h,i,j,k,l,m,n,o,p,q,r,t,u,v,w,x,y,z }

\clist_new:N \g_fouche_both_clist
\clist_concat:NNN \g_fouche_both_clist \g_fouche_upper_clist \g_fouche_lower_clist

\clist_new:N \g_fouche_categories_clist
\clist_gset:Nn \g_fouche_categories_clist { Ab, Alg, Ban, BSD, Card, cat, Cat, CAT, cgHaus, Ch, CMnd, CMon, CW, Der, EM, End, Ext, fHilb, Fld, Foo, Fuk, fVect, Fzy, Gal, Grp, gVec, Haus, Het, Ho, Kl, Lat, Mag, Met, Mfd, Mnd, Mod, Mon, Ord, Par, PInj, POrd, Pre, Pro, Prof, Quot, Quux, Rel, Ring, Rot, Set, Sgp, Sp, Spec, sSet, Sub, SW, Top, Tor, Unif, Vect }

\clist_new:N \g_fouche_operators_clist
\clist_gset:Nn \g_fouche_operators_clist { lan, Lan, LAN, lft, Lft, LFT, Nat, ran, Hom, Ran, RAN, Rft, Yan,RFT, rft, op, co, coop, colim, coker, }

\cs_new_protected:Npn \fouche_makeabbrev:nnN #1 #2 #3
 {
  \clist_map_inline:Nn { #3 }
   {
    \cs_new_protected:cpn { #2 } { #1 { ##1 } }
   }
 }
\fouche_makeabbrev:nnN { \textbf } { bf#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \boldsymbol } { bs#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \textsf } { sf#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \mathfrak } { fk#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \underline } { un#1 } \g_fouche_both_clist

\fouche_makeabbrev:nnN { \mathcal } { cl#1 } \g_fouche_upper_clist
\fouche_makeabbrev:nnN { \mathbb } { bb#1 } \g_fouche_upper_clist

\fouche_makeabbrev:nnN { \textsf } { #1 } \g_fouche_categories_clist
\fouche_makeabbrev:nnN { \mathrm } { #1 } \g_fouche_operators_clist

\DeclareMathAlphabet{\mybb}{U}{BOONDOX-ds}{m}{n}
\fouche_makeabbrev:nnN { \mybb } { mb#1 } \g_fouche_lower_clist
\ExplSyntaxOff


==> fouche/envs.tex <==
\DeclareOption{english}{
\theoremstyle{definition}
\numberwithin{equation}{section}
\newtheorem{theorem}{Theorem}[section]
 \defthm{corollary}{Corollary}
 \defthm{proposition}{Proposition}
 \defthm{lemma}{Lemma}
 \defthm{claim}{Claim}
 \defthm{definition}{Definition}
 \defthm{notation}{Notation}
 \defthm{remark}{Remark}
 \defthm{conjecture}{Conjecture}
 \defthm{axiom}{Axiom}
 \defthm{example}{Example}
 \defthm{examples}{Examples}
 \defthm{exercise}{Exercise}
 \defthm{counterexample}{Counterexample}
 \defthm{construction}{Construction}
 \defthm{warning}{Warning}
 \defthm{digression}{Digression}
 \defthm{perspective}{Perspective}
 \defthm{discussion}{Discussion}
 \defthm{terminology}{Terminology}
 \defthm{heuristics}{Heuristics}
 \defthm{conclusion}{Conclusion}
}

\makeatletter
\def\renewtheorem#1{%
  \expandafter\let\csname#1\endcsname\relax
  \expandafter\let\csname c@#1\endcsname\relax
  \gdef\renewtheorem@envname{#1}
  \renewtheorem@secpar
}
\def\renewtheorem@secpar{\@ifnextchar[{\renewtheorem@numberedlike}{\renewtheorem@nonumberedlike}}
\def\renewtheorem@numberedlike[#1]#2{\newtheorem{\renewtheorem@envname}[#1]{#2}}
\def\renewtheorem@nonumberedlike#1{
\def\renewtheorem@caption{#1}
\edef\renewtheorem@nowithin{\noexpand\newtheorem{\renewtheorem@envname}{\renewtheorem@caption}}
\renewtheorem@thirdpar
}
\def\renewtheorem@thirdpar{\@ifnextchar[{\renewtheorem@within}{\renewtheorem@nowithin}}
\def\renewtheorem@within[#1]{\renewtheorem@nowithin[#1]}
\makeatother

\makeatletter
\def\redefthm#1#2{%
  \renewtheorem{#1}{#2}[section]%
  \expandafter\def\csname #1autorefname\endcsname{#2}%
  \expandafter\let\csname c@#1\endcsname\c@theorem}
\makeatother

\DeclareOption{italian}{
\theoremstyle{definition}
\numberwithin{equation}{section}
\renewtheorem{theorem}{Teorema}[section]
 \redefthm{corollary}{Corollario}
 \redefthm{proposition}{Proposizione}
 \redefthm{lemma}{Lemma}
 \redefthm{definition}{Definizione}
 \redefthm{notation}{Notazione}
 \redefthm{remark}{Osservazione}
 \redefthm{conjecture}{Congettura}
 \redefthm{axiom}{Assioma}
 \redefthm{example}{Esempio}
 \redefthm{examples}{Esempi}
 \redefthm{exercise}{Esercizio}
 \redefthm{exercises}{Esercizi}
 \redefthm{counterexample}{Controesempio}
 \redefthm{construction}{Costruzione}
 \redefthm{warning}{Caveat}
 \redefthm{digression}{Digressione}
 \redefthm{perspective}{Prospettiva}
 \redefthm{discussion}{Discussione}
 \redefthm{terminology}{Terminologia}
 \redefthm{heuristics}{Euristica}
}

\DeclareDocumentEnvironment{enumtag}{m O{}}{%
	\begin{enumerate}[ label = \textsc{#1}\oldstylenums{\arabic*}), ref   = \textsc{#1}\oldstylenums{\arabic*}, #2] }{ \end{enumerate} }


==> fouche/macros.tex <==
\def\To{\Rightarrow}

\newcommand{\arXivPreprint}[1]{\href{http://arxiv.org/abs/#1}{arXiv:#1} preprint}

\newlength{\seplen}
\setlength{\seplen}{5pt}
\newlength{\sepwid}
\setlength{\sepwid}{.4pt}
\def\firstblank{\,\rule{\seplen}{\sepwid}\,}
\def\sndblank{\firstblank\llap{\raisebox{2pt}{\firstblank}}}

\newcommand{\celtag}[2][dr]{\ar[#1,white, "#2"{black,description}]}


\let\xto\xrightarrow
\let\xot\xleftarrow

\newcommand{\rot}[3][c]{\rotatebox[origin=#1]{#2}{$#3$}}
\newcommand{\rotarrow}[2][c]{\rot{#1}{#2}{\Rightarrow}}

\newcommand{\Nearrow}{\rotarrow{45}}
\newcommand{\Nwarrow}{\rotarrow{135}}
\newcommand{\Searrow}{\rotarrow{-45}}
\newcommand{\Swarrow}{\rotarrow{225}}
\newcommand{\Sarrow}{\rotarrow{-90}}
\newcommand{\Narrow}{\rotarrow{90}}

\newcommand{\bsmat}{\begin{smallmatrix}}
\newcommand{\esmat}{\end{smallmatrix}}

\makeatletter
  \def\@cite#1#2{[\textsf{#1}\if@tempswa , #2\fi]}
  \def\@biblabel#1{[\textsf{#1}]}
\makeatother


\newcommand{\pto}{\mathop{\ooalign{\hfil\kern-2pt$\mapstochar$\hfil\cr\hfil$\to$\hfil}}}

\usepackage{turnstile}
\newcommand{\adjunct}[2]{\nsststile{#2}{#1}}

\newcommand{\putbib}[2]{
  \bibliography{#1}{}
  \bibliographystyle{#2}
}

\usetikzlibrary{decorations.markings}
\tikzstyle{pro} =
  [ decoration={ markings
               , mark = at position 0.5 with
                   {\draw[-] (0,-1.25pt) -- (0,1.25pt);}
               }
  , postaction ={decorate}
  ]

\newcommand*{\Scale}[2][4]{\scalebox{#1}{\ensuremath{#2}}}%
\def\lrc{
\begin{tikzpicture}[scale=.33]
	\draw[-] (0,0) -| (1,1);
\end{tikzpicture}
}

\def\dopb{\begin{tikzpicture}[scale=.375] \draw (0,0) -| (1,1);\end{tikzpicture}}
\newcommand{\xpb}[1][dr]{\ar@{}[#1]|(.375){\dopb}}
\def\dopo{\begin{tikzpicture}[scale=.375] \draw (0,0) |- (1,1);\end{tikzpicture}}
\newcommand{\xpo}[1][dr]{\ar@{}[#1]|(.675){\dopo}}

\newcommand{\pb}{\arrow[dr, phantom, "\dopb", very near start]}
\newcommand{\po}{\arrow[dr, phantom, "\dopo", very near end]}

\def\[{\begin{equation}}
\def\]{\end{equation}}
% ^ this is BAD, but can't do without at this point...

\newenvironment{xsmallmatrix}[1]
{\renewcommand\thickspace{\kern#1}\smallmatrix}
{\endsmallmatrix}

\NewDocumentCommand{\prevar}{o m m}{
	\IfNoValueTF{#1}{
			\begin{smallmatrix}
				#2 \\
				\downarrow \\
				#3
			\end{smallmatrix}}
	{
			\begin{xsmallmatrix}{0em}
				& #2 \\
				#1 & \downarrow \\
				& #3
			\end{xsmallmatrix}}}

\ExplSyntaxOn
\NewDocumentCommand{\var}{o m O{s} m}{
	\str_case:nn { #3 } {
		{r}{\left( \prevar[#1]{#2}{#4}\right)}
		{s}{\left[ \prevar[#1]{#2}{#4}\right]}
		{c}{\left\{ \prevar[#1]{#2}{#4}\right\}}
		{a}{\left\langle \prevar[#1]{#2}{#4}\right\rangle}
	}}
	\newcommand{\precop}[2]{
		\begin{smallmatrix}
			#1 \\ #2
		\end{smallmatrix}
	}
	\NewDocumentCommand{\cop}{O{r} m m}{
		\str_case:nn { #1 } {
			{r}{\left( \precop{#2}{#3}\right)}
			{s}{\left[ \precop{#2}{#3}\right]}
			{c}{\left\{ \precop{#2}{#3}\right\}}
			{a}{\left\langle \precop{#2}{#3}\right\rangle}
		}}

\ExplSyntaxOff

\usepackage{adjustbox}
\newenvironment{adju}[1][0.925]{%
\begin{center}\begin{adjustbox}{max height=0.5\textheight, max width=#1\textwidth}}{\end{adjustbox}\end{center}}

\def\emdash{\text{-}}
\NewDocumentCommand{\VCat}{ O{\clV} }{#1\emdash\Cat}
\def\twoCat{\VCat[2]}

\newcommand{\adja}[4]{
  #1 : \xymatrix{#2 \ar@<.5em>[r] \ar@{}[r]|\perp & \ar@<.5em>[l] #3 } : #4
}


\NewDocumentCommand{\vxy}{o m}{
  \IfNoValueTF{#1}
  {\vcenter{\xymatrix{#2}}} % do if \vxy{bla}
  {\vcenter{\xymatrix#1{#2}}} % do if \vxy[foo]{bla}
}

==> fouche/packages.tex <==

\RequirePackage{amsthm}
\RequirePackage[svgnames]{xcolor}
\RequirePackage{ amsfonts
               , amsmath
               , amssymb
               , caption
               , epigraph
               , enumitem
               , lipsum
               , mathtools
               , hyphenat
               , tensor
               , todonotes
               , stackrel
               , tikz
               , hyperref
               , savesym
               , setspace
               , tikz-cd
               , tcolorbox
               , verbatim
               , calligra
               , url
               }
\RequirePackage[all,2cell]{xy}\UseAllTwocells

% setup of specific packages

\usetikzlibrary{calc}
\usetikzlibrary{matrix,arrows}

\hypersetup{ hyperfootnotes=true%
	         , bookmarksnumbered=true%
	         , bookmarksopen=true%
	         , breaklinks=true%
	         , urlcolor=black%
	         , colorlinks%
	         , citecolor=black%
	         , linkcolor=black%
	         , urlcolor=black%
           }

\tikzset{commutative diagrams/.cd,arrow style=tikz,diagrams={>=stealth'}}


==> fouche/page-layout.tex <==
%per le formule nei titoli
%-------------------------------------------------------------------------
\makeatletter
\g@addto@macro\bfseries{\boldmath}
\makeatother
%-------------------------------------------------------------------------

\makeatletter
\def\defthm#1#2{%
  \newtheorem{#1}{#2}[section]%
  \expandafter\def\csname #1autorefname\endcsname{#2}%
  \expandafter\let\csname c@#1\endcsname\c@theorem}
\makeatother

\tcbuselibrary{most}
\tcolorboxenvironment%
  {quote}{ blanker
         , before skip=10pt
         , after skip=10pt
         , borderline west={6mm}{5pt}{gray!15}
         , breakable
         }

\setcounter{tocdepth}{1}


==> secs/04-furtherNotions.tex <==
\section{Further notions of composition}
%
%
In this section, we explore other ways to compose escrows with each other. In~[], we came up with a notion of composition that uses $B$ as an intermediary in the transaction betwen $A$ and $C$. In that model, $B$ could be considered "greedy" as she cashes in her escrow before $C$, the final producer, does. So $C$ has to wait for the whole procedure to be finished to receive her payment.

In the following, we model a different notion of composition that we name \emph{kind}: $B$ will release her escrow to $C$ upon receiving the goods, and only then settle with $A$:
%
%
%
%
\begin{equation*}
	%
	%
	%
	\begin{tikzpicture}
		\up[2]{\gau{$A$}}
		\yScale{\arTwo[green!10]{$\faLock$}}
		\step{
			\node[below, font=\tiny] at (0,2*\nlen) {$B$};
			\up[4]\idn
			\arTwo[green!10]{$\faLock$}
			\down{\dro{$C$}}
			\step[0.5]{\down{\dro{$B$}}}
		}
		\step[2]{
			\up[4]{
				\idn
				\step{\node[below, font=\tiny] at (0,2*\nlen) {$E_1$};}
			}
			\up[1]{
				\idn
				\step[0.5]{\node[below, font=\tiny] at (0,2*\nlen) {$E_2$};}
			}
		}
		\step[3]{
			\twoAr[green!10]{$\faUnlock$}
			\up[4]\idn
			\step{
				\up[4]\idn
				\node[below, font=\tiny] at (0,2*\nlen) {$C$};
			}
			\step[2]{
				\node[below, font=\tiny] at (0,2*\nlen) {$A$};
				\yScale{\twoAr[green!10]{$\faUnlock$}\dro{$B$}}
			}
		}
	\end{tikzpicture}
	%
	\hspace{6em}
	\begin{tikzpicture}
		\gau{$C$}\mor[red!10, minimum height=12, minimum width=12]{$\faEnvelope$}
		\step{\node[below, font=\tiny] at (0,2*\nlen) {$B$};}
		\down[3]{
			\gau{$C$}\mor[red!10, minimum height=12, minimum width=12]{$\faEnvelope$}
			\step{\node[below, font=\tiny] at (0,2*\nlen) {$B$};}
			\step{\mor[red!10, minimum height=12, minimum width=12]{$\faEnvelope$}\dro{$A$}}
		}
	\end{tikzpicture}
\end{equation*}
%
By looking at the combs, it is clear that the transaction $C \to B$, representing the delivery of goods from $C$ to $B$, must be used to times: The first time to release the escrow from $B$ to $C$, while the second time, composed with $B \to A$ to release the escrow from $A$ to $B$. Using coend calculus,
%
%
\begin{equation*}
	MORE \quad COEND \quad MAGIC
\end{equation*}
%


==> secs/06-app.tex <==
\appendix
\section{Appendix: proofs}
\begin{proof}[Proof of \cref{pf:assoc}]
	Associativity: suppose given a triple $(h,k,p)$ such that
	\[
		h = \left(
		\begin{tikzpicture}[baseline=(current bounding box.center)]
				\arTwo[magenta!10]{h_1}
			\end{tikzpicture}\, , \,
		\begin{tikzpicture}[baseline=(current bounding box.center)]
				\twoAr[blue!10]{h_2}
			\end{tikzpicture}
		\right)\quad
		k =   \left(  \begin{tikzpicture}[baseline=(current bounding box.center)]
				\arTwo[teal!10]{k_1}
			\end{tikzpicture}\, , \,
		\begin{tikzpicture}[baseline=(current bounding box.center)]
				\twoAr[yellow!10]{k_2}
			\end{tikzpicture} \right)\quad
		p =   \left(
		\begin{tikzpicture}[baseline=(current bounding box.center)]
				\arTwo[orange!10]{p_1}
			\end{tikzpicture}\, , \,
		\begin{tikzpicture}[baseline=(current bounding box.center)]
				\twoAr[cyan!10]{p_2}
			\end{tikzpicture}
		\right)
	\]
	In string diagram notation, the two possible compositions of $h,k,p$ are given, respectively, by the following pairs:
	\[
		\underset{(h\diamond k)\diamond p}{\left( \begin{tikzpicture}[scale=.5,baseline=(current bounding box.center)]
				\yScale[3]{\arTwo[orange!10]{}}
				\down{\yScale{\step{\arTwo[teal!10]{}\xScale{\up[3]\idn}}}
					\step[2]{\arTwo[magenta!10]{}\up[4]\idn}}
			\end{tikzpicture}
			\,,\,
			\begin{tikzpicture}[scale=.75]
				\step[-1]{\up[3.5]\twoid}
				\down[.5]{\step[-1]{\yScale[3]\coturn}
					\twoAr[cyan!10]{}}
				\up[3.5]{\braid}
				\step{\yScale[1.5]{\twoAr[yellow!10]{}}}
				\step[2]{\up[1.25]{\yScale[1.75]{\twoAr[blue!10]{}}}}
				\step{\up[4.5]\idn}
				\step[-1]{\down[1.5]\idn}
			\end{tikzpicture}
			\right)}
		\qquad
		\underset{h\diamond (k\diamond p)}{\left(
			\begin{tikzpicture}[scale=.5,baseline=(current bounding box.center)]
				\yScale[3]{\arTwo[orange!10]{}}
				\down{\yScale{\step{\arTwo[teal!10]{}\xScale{\up[3]\idn}}}
					\step[2]{\arTwo[magenta!10]{}\up[4]\idn}}
			\end{tikzpicture}
			\,,\,\begin{tikzpicture}[scale=.75]
				\down[.5]{\up[3]\idn\twoAr[cyan!10]{}}
				% \up[3.5]{\braid}
				\step{\yScale[1.5]{\twoAr[yellow!10]{}}}
				\step[2]{\up[1.25]{\yScale[1.75]{\twoAr[blue!10]{}}}}
				\step{\up[4.5]\idn}
				\step[-1]{\up[1.5]{\braid}\down[1.5]\idn}
				\up[1.5]{\step[-1]{\draw[wire] (0,0) -| (1,1.25) -- ++(1,0);}}
			\end{tikzpicture}
			\right)}
	\]
	Unitality: define $\nu_S$, as the equivalence class of the pair $(\lambda^{-1},\rho)$ in the coend
	\[\label{aoaou}\int^M \clM(S,M\otimes S)\times \clM(M\otimes S,S)\]
	(more formally, consider the summand at $M=I$ --the monoidal unit; the product of hom sets
	\[\clM(S,I\otimes S)\times \clM(I\otimes S,S)\]
	contains the element $\left(\var{S}{I\otimes S},\var{I\otimes S}{S}\right)$ obtained from the unitors of the monoidal structure; now project on the quotient that defines the coend in Equation \eqref{aoaou}) and use a straightforward string diagrammatic argument.
\end{proof}

\begin{proof}[Proof of \cref{itsa_monoid}]
  One routinely checks the associativity and unit axioms from the following definitions:
  \begin{itemize}
    \item given two escrows $(h_1,h_2)$ and $(k_1,k_2)$ as in
          \[
            \esc{A}{h}{C} \qquad \esc[teal][yellow]{A}{k}{C}[N]
          \]
          we compose them into the escrow $h\otimes k$
          \[
            \begin{tikzpicture}
              \yScale{\comult}
              \step{\up[4]{\arTwo[magenta!10]{h_1}}\arTwo[teal!10]{k_1}}
              \step[2]{\up[4]{\xScale[3]\Uid}\up[2]\turn\down{\yScale{\mult}}}
              \step[3]{\up[3]\idn}
              \step[4]{
                \down{\yScale{\comult}\up[3]\coturn}
                \step{\up[4]{\twoAr[blue!10]{h_2}}\twoAr[yellow!10]{k_2}}
                \step[2]{\yScale{\mult}}
              }
            \end{tikzpicture}
          \]
          using the monoid and comonoid structures of $C, A$ respectively;
    \item the unit escrow $(i_1,i_2)$ is the lower morphism in
          \[
            \begin{tikzpicture}
              \down[2.5]{\yScale[1.5]{\step[-1]{\comult}}}
              \arTwo[magenta!10]{h_1} \down[3]{\counit \down[2]\unit}\step[4]{\twoAr[blue!10]{h_2} \down[3]{\unit \down[2]\counit}}
              \down[5]{\step{\yScale{\mult}} \step[3]{\yScale{\comult}}}
              \down[2.5]{\yScale[1.5]{\step[5]{\mult}}}
              \step{\up{\xScale[3]\idn}}
              \down[4]\akasa \step[4]{\down[4]\akasa}
              \node at (.5,-.5) {\tiny $i_1$};
              \node at (4.5,-.5) {\tiny $i_2$};
            \end{tikzpicture}
          \]
          obtained using the counit of $A$ and the unit of $C$. Evidently, the co/monoid rules entail that $h\otimes i$ is just equal to $h$, for every other optic $h=(h_1,h_2)$. Similarly, one sees that $i\otimes k=k$. \qedhere
  \end{itemize}
\end{proof}

\begin{proof}[Proof of \cref{escaction}]
  Suppose given an escrow and an optic, as the following pairs:
  \[
    \left(
    \begin{tikzpicture}[baseline=(current bounding box.center)]
        \arTwo[magenta!10]{h_1}\gau{$A$}\down{\dro{$C$}}
      \end{tikzpicture}\, , \,
    \begin{tikzpicture}[baseline=(current bounding box.center)]
        \twoAr[blue!10]{h_2}\dro{$C$}\down{\gau{$A$}}
      \end{tikzpicture}
    \right) \qquad
    \left(
    \begin{tikzpicture}[baseline=(current bounding box.center)]
        \arTwo[teal!10]{o_1}\gau{$A$}\down{\dro{$B$}}
      \end{tikzpicture}\, , \,
    \begin{tikzpicture}[baseline=(current bounding box.center)]
        \twoAr[yellow!10]{o_2}\dro{$C$}\down{\gau{$B$}}
      \end{tikzpicture}
    \right)
  \]
  Now define the action as follows:
  \[
    \begin{tikzpicture}
      \yScale{\comult}%\coact{$c$}}
      \step{\up[4]{\arTwo[magenta!10]{h_1}}\arTwo[teal!10]{o_1}}
      \step[2]{\up[4]{\xScale[3]\Uid}\down{\yScale{\act{$a$}}}}
      % \step[3]{\up[3]\idn}
      \step[4]{
        \down{\yScale{\coact{$c$}}}
        \step{\up[4]{\twoAr[blue!10]{h_2}}\twoAr[yellow!10]{o_2}}
        \step[2]{\yScale{\mult}}
      }
      \draw[wire] (2,3*\nlen) -| ++(.15,3*\nlen) -| ++(2.75,-.75) |- ++(.15,0);
    \end{tikzpicture}
  \]
  using the monoid structure of $C$, comonoid structure of $A$, module and comodule structure of $B$. We shall now prove the axioms of an action:
  \begin{enumerate}
    \item \label{a_1} \emph{unitality} axiom: the fact that $i\rtimes o=o$ for every optic $o=(o_1,o_2)$ and for the unit escrow $i\in\lr A C $.
    \item \label{a_2} the \emph{action} axiom, saying that $(k\otimes h) \rtimes o = k  \rtimes (h \rtimes o)$ for escrows $h,k$ and an optic $o$.
  \end{enumerate}
  Axiom \ref{a_1} follows from a simple string diagram deformation, using the unit axiom of the co/monoid and co/action structures:
  \[
    \begin{tikzpicture}[xscale=.75]
      \step{\up[3]\akasa}
      \yScale{\comult}
      \step{\up[4]{\counit\down[2]\unit}\arTwo[teal!10]{o_1}}
      \step[2]{\down[.5]{\yScale[1.5]{\act{$a$}}}\up[2]\turn}
      \step[4]{
        \step{\up[3]\akasa}
        \down[.5]{\yScale[1.5]{\coact{$c$}}\up[2.5]\coturn}
        \step{\up[4]{\unit\down[2]\counit}\twoAr[yellow!10]{o_2}}
        \step[2]{\yScale{\mult}}
      }
      \step[3]{\up[3]\idn}
      \begin{scope}[xshift=7.5cm]
        \yScale{\comult}
        \step{\up[4]{\counit}\arTwo[teal!10]{o_1}}
        \step[2]{
          \step{\up[4]{\unit}\twoAr[yellow!10]{o_2}}
          \step[2]{\yScale{\mult}}
        }
        \up{\step[2]\idn}
      \end{scope}
      \begin{scope}[xshift=13cm,yshift=.5cm]
        \arTwo[teal!10]{o_1}
        \step{\up\idn}
        \step[2]{\twoAr[yellow!10]{o_2}}
      \end{scope}
    \end{tikzpicture}
  \]
  Similarly, axiom \ref{a_2} follows from the co/associativity of the co/action and co/multiplication applied to the following equality of wire diagrams, where on the left we have $k\rtimes (h\rtimes o)$ (slightly simplifying its structure to avoid cognitive overload), and on the right $(k\otimes h)\rtimes o$:
  \[
    \begin{tikzpicture}[xscale=.75]
      \step[-1.5]{\down[4.75]{\yScale[2.25]\comult}}
      \step[-.5]{\down[5.5]{\xScale[.5]{\yScale[1.5]\comult}}\xScale[.5]\idn}
      \arTwo[orange!10]{k_1}
      \down[3]{\arTwo[magenta!10]{h_1}}
      \down[6]{\arTwo[teal!10]{o_1}}
      \step{\up{\xScale\idn}}
      \step{\down[2]{\xScale\idn}}
      \step{\down[5]{\xScale\idn}}
      \step[3]{
        \twoAr[cyan!10]{k_2}
        \down[3]{\twoAr[blue!10]{h_2}}
        \down[6]{\twoAr[yellow!10]{o_2}}
        \step{\down[5.5]{\xScale[.5]{\yScale[1.5]\mult}}\xScale[.5]\idn}
        \step[1.5]{\down[4.75]{\yScale[2.25]\mult}}
      }
      \draw[wire] (1,-1.25) -| ++(\nlen,3*\nlen) -- ++(-\nlen,0);
      \draw[wire] (1.25,-1) -| ++(.5,5*\nlen) -- ++(-3*\nlen,0);
      \draw[wire] (3,-1.25) -| ++(-\nlen,3*\nlen) -- ++(\nlen,0);
      \draw[wire] (2.75,-1) -| ++(-.5,5*\nlen) -- ++(3*\nlen,0);
    \end{tikzpicture}
    \quad
    %%%%%
    \begin{tikzpicture}[xscale=.75]
      \step[-1.5]{\down[6.25]{\yScale[2.25]\comult}}
      \step[-.5]{\down[2.5]{\xScale[.5]{\yScale[1.5]\comult}}\down[6]{\xScale[.5]\idn}}
      \arTwo[orange!10]{k_1}
      \down[3]{\arTwo[magenta!10]{h_1}}
      \down[6]{\arTwo[teal!10]{o_1}}
      \step{\up{\xScale\idn}}
      \step{\down[2]{\xScale\idn}}
      \step{\down[5]{\xScale\idn}}
      \step[3]{
        \twoAr[cyan!10]{k_2}
        \down[3]{\twoAr[blue!10]{h_2}}
        \down[6]{\twoAr[yellow!10]{o_2}}
        \step{\down[2.5]{\xScale[.5]{\yScale[1.5]\mult}}\down[6]{\xScale[.5]\idn}}
        \step[1.5]{\down[6.25]{\yScale[2.25]\mult}}
      }
      \up[3]{\draw[wire] (1,-1.25) -| ++(\nlen,3*\nlen) -- ++(-\nlen,0);}
      \down{\draw[wire] (1,-1) -| ++(.5,4*\nlen) -- ++(-\nlen,0);}
      \up[3]{\draw[wire] (3,-1.25) -| ++(-\nlen,3*\nlen) -- ++(\nlen,0);}
      \down{\draw[wire] (3,-1) -| ++(-.5,4*\nlen) -- ++(\nlen,0);}
    \end{tikzpicture}
  \]
  This concludes the proof.
\end{proof}

\begin{proof}[Proof of \cref{Vermittler}]
  Recall from \cite[4.13]{2001.07488} that the hom-set $\Opt(\cop AB, \cop ST)$ can be expressed as the end
  \[\int_P \hom(P(A,B), P(S,T))\label{dis_tamba}\]
  where $P : \clM^\op\times \clM \to \Set$ is a profunctor, and the category of integration is that  of Tambara modules \cite[4.1]{2001.07488}. Now,
  \begin{itemize}
    \item the fact that $P$ is a Tambara module yields maps
          \[\xymatrix{\alpha_{[B]}^{AC} : P(C,A) \ar[r] & P(C\otimes B, A\otimes B)}\]
          that form a wedge in $B$; post-composition with these $\alpha_{[B]}^{AC}$ and the universal wedge $\pi^\bullet$ defining Equation \eqref{dis_tamba} yields maps
          \[\xymatrix{
            \lr CA \ar@{=}[r]&\int_Q \hom(Q(A,C), Q(C,A))\ar[dr]_{\tilde\alpha_P} \ar[r]^{\pi^P} & \hom(P(A,C), P(C,A)) \ar[d]^{\alpha_{[B],*}^{AC}}\\
            && \hom(P(A,C), P(C\otimes B, A\otimes B))
            }\]
          forming a wedge in $P$. This in turn yields a unique map
          \[\xymatrix{\tilde\alpha : \lr CA \ar[r] & \clV(B;A,C)}\]
          by the universal property of the end that defines $\clV(B;A,C)$.
    \item The assumption that $B$ is at the same time a module for the monoid $C$ and a comodule for the comonoid $A$ entails the existence of an action map $a : C\otimes B \to B$ and a coaction map $c : B \to A\otimes B$, which plugged into the profunctor $P$ yield
          \[\xymatrix{\beta_{[B]}^{AC} = P(a,c) : P(B,B) \ar[r] & P(C\otimes B, A\otimes B).}\]
          In a similar fashion, post-composition with $\beta_{[B]}^{AC}$, and the universal property of the end defining domain and codomain of $\tilde\beta$ define such a map as
          \[\tilde\beta : \xymatrix{\Opt(\cop CA, \cop BB)\ar[r] & \clV(B;A,C)}\]
          so that we obtain a cospan of maps
          \[\xymatrix{
              & \lr CA\ar[d]^{\tilde\alpha}\\
              \Opt(\cop CA, \cop BB)\ar[r]_{\tilde\beta} & \clV(B;A,C),
            }\]
          and we can consider its pullback $Z$ (in $\Set$, or inside a sufficiently cocomplete ambient category). The diagonal in the pullback is the candidate partial function
          \[
            \xymatrix{
              &Z \ar[dr]\ar[dl]& \\
              \lr CA\times \Opt(\cop CA, \cop BB) \ar@{.>}[rr]_-\lhd && \clV(B;A,C)
            }
          \]
          having $Z$ as its domain of definition. As such, $k\lhd f$ is defined as soon as $\tilde\alpha(k)=\tilde\beta(f)$, and it equals any of these two elements.
  \end{itemize}
  The main intuition behind this construction is the following: the object $Z$ is the maximal subobject of the product $\lr CA\times \Opt(\cop CA, \cop BB)$ with the property that the conjoint action and coaction over $B$, and all actions given by the Tambara module structure maps $\alpha^B$, agree. This yields a unique partial map $\firstblank \lhd \firstblank$
  % \[\xymatrix{\lhd : \lr AC \times  \Opt(\cop AC, \cop BB) \ar[r] & \Opt(\cop AC, \cop{C\times B}{A\times B}) }\]
  that defines a \emph{partial action} of the monoid $\lr AC$ on the set of Vermittler optics over $B$.

  It only remains to show that this map satisfies the commutativities of \eqref{questa} and \eqref{laltra} when the domain of $\lhd$ has been suitably defined as above; to argue equationally, with the definition and the universal properties of $Z$ and the hom-sets of optics, is certainly possible but rather unwieldy. Instead, the following remark will give a graphical interpretation of the above partial action that makes the action axioms almost tautological. This will conclude the proof.
\end{proof}

\begin{remark}
  We can give a concise graphical representation of the action of the maps $\tilde\alpha,\tilde\beta$ above:
  \begin{itemize}
    \item the map $\tilde\alpha$ acts sending an escrow
          \[\left(
            \begin{tikzpicture}[baseline=(current bounding box.center)]
                \arTwo[magenta!10]{h_1}\gau{$C$}\down{\dro{$A$}}
              \end{tikzpicture}\, , \,
            \begin{tikzpicture}[baseline=(current bounding box.center)]
                \twoAr[blue!10]{h_2}\dro{$A$}\down{\gau{$C$}}
              \end{tikzpicture}
            \right)\]
          to the `trivial' Vermittler optic obtained by tensoring with the identity arrow $1_B$:
          \[\alpha(h) =\quad
            \left(
            \begin{tikzpicture}[baseline=(current bounding box.center)]
                \arTwo[magenta!10]{h_1}\gau{$C$}\down{\dro{$A$}}
                \down[3]{\idn\dro{$B$}\gau{$B$}}
              \end{tikzpicture}\, , \,
            \begin{tikzpicture}[baseline=(current bounding box.center)]
                \twoAr[blue!10]{h_2}\dro{$A$}\down{\gau{$C$}}
                \down[3]{\idn\dro{$B$}\gau{$B$}}
              \end{tikzpicture}
            \right)\]
    \item the map $\tilde\beta$ acts sending an optic $\cop CA \to \cop BB$ to the Vermittler optic obtained by plugging in the action and coaction map of $A,C$ over $B$:
          \[\tilde\beta(o) =\quad
            \left(
            \begin{tikzpicture}[xscale=.75,baseline=(current bounding box.center)]
                \act{$a$}\down{\gau{$B$}}\up{\gau{$C$}}
                \step{\arTwo[green!10]{o_1}\down{\dro{$A$}}}
              \end{tikzpicture}\, , \,
            \begin{tikzpicture}[xscale=.75,baseline=(current bounding box.center)]
                \twoAr[yellow!10]{o_2}\down{\gau{$C$}}
                \step{\coact{$c$}\up{\dro{$A$}}\down{\dro{$B$}}}
              \end{tikzpicture}
            \right)\]
  \end{itemize}
\end{remark}
